Online Data Collection for Efficient Semiparametric Inference

While many works have studied statistical data fusion, they typically assume that the various datasets are given in advance. However, in practice, estimation requires difficult data collection decisions like determining the available data sources, their costs, and how many samples to collect from each source. Moreover, this process is often sequential because the data collected at a given time can improve collection decisions in the future. In our setup, given access to multiple data sources and budget constraints, the agent must sequentially decide which data source to query to efficiently estimate a target parameter. We formalize this task using Online Moment Selection, a semiparametric framework that applies to any parameter identified by a set of moment conditions. Interestingly, the optimal budget allocation depends on the (unknown) true parameters. We present two online data collection policies, Explore-then-Commit and Explore-then-Greedy, that use the parameter estimates at a given time to optimally allocate the remaining budget in the future steps. We prove that both policies achieve zero regret (assessed by asymptotic MSE) relative to an oracle policy. We empirically validate our methods on both synthetic and real-world causal effect estimation tasks, demonstrating that the online data collection policies outperform their fixed counterparts.

==> sections/additional-settings.tex <==
\begin{enumerate}
    \item Proxy setting with two data sources:
    (1) the first data sources gives $\{ Z, X, Y \}$, and
    (2) the second source gives $\{ W, Z \}$, where
    $W$ is a confounder and $Z$ is a proxy of the confounder
    (use the effect restoration formula).
    Not sure if the semiparametric estimator is known in this setting.
\end{enumerate}

Some possible datasets
\begin{enumerate}
    \item Neuropathic Pain Diagnosis Simulator for Causal Discovery Algorithm Evaluation
    \item Transporting Causal Effects Across Populations Using Structural Causal Modeling:An Illustration to Work-From-Home Productivity
    \item HowandWhytoUseExperimentalDatatoEvaluateMethodsforObservationalCausalInference
    \item 
\end{enumerate}
